Gaze-Contingent Ocular Parallax Rendering for Virtual Reality

Immersive computer graphics systems strive to generate perceptually realistic user experiences. Current-generation virtual reality (VR) displays are successful in accurately rendering many perceptually important effects, including perspective, disparity, motion parallax, and other depth cues. In this article, we introduce ocular parallax rendering, a technology that accurately renders small amounts of gaze-contingent parallax capable of improving depth perception and realism in VR. Ocular parallax describes the small amounts of depth-dependent image shifts on the retina that are created as the eye rotates. The effect occurs because the centers of rotation and projection of the eye are not the same. We study the perceptual implications of ocular parallax rendering by designing and conducting a series of user experiments. Specifically, we estimate perceptual detection and discrimination thresholds for this effect and demonstrate that it is clearly visible in most VR applications. Additionally, we show that ocular parallax rendering provides an effective ordinal depth cue and it improves the impression of realistic depth in VR.

==> sections/supplement_disparity.tex <==
% !TeX root = ../supplement.tex



In Figure~\ref{fig:supp:disparity}, we show additional details for calculating the disparity distortions of objects in the periphery of the visual field. On the right, we illustrate the settings we simulated: a user fixating on the optical axis on one of four different depths, either 1~D (1~m), 2~D (50~cm), 3~D (33.3~cm), or 4~D (25~cm). For each of these fixation distances, we then traced out points with the same respective distance from the center point between the eyes along an arc (red points). We then calculated what the disparity angles to left and right eye would be when rays go directly from the individual points through the center of rotation of the eyes and when they go through the front nodal point. The discrepancy between these disparity angles is plotted for all four distance settings and for a range of eccentricity angles (i.e., points moving along the arc) in the left. We see that the disparity distortion is zero for foveal vision, but steadily increases the farther we go into peripheral vision. Although the disparity distortion measured in angles of visual degrees is more pronounced for closer distances, when converting these distortion to meters, they are fairly independent of depth (center). However, the maximum depth distortion is only about 4~mm at an eccentricity of $60^{\circ}$, which is negligible. The perceived location of the distorted points is also rendered by blue dots on the right, showing that they are fairly close to the target points. 

While these distortions increase in the periphery, they may not be perceptible because stereoacuity also decreases in the periphery~\cite{Rawlings:69,McKee:83}. For example, stereoacuity at 10\textdegree\ eccentricity was measured to be 80~arcsec~\cite{Fendick:83}. In comparison, the expected amount of disparity distortion due to a lack of appropriate ocular parallax rendering at 10\textdegree\ eccentricity is 73.76 arcsec (fixating at 4~D). This implies that the disparity distortions of conventional stereo rendering in peripheral vision may be too small to have a measurable effect on depth perception, which was indeed verified by the egocentric distance estimation study in the main paper. However, the micro parallax and gaze-contingent occlusion induced by ocular parallax rendering were shown to improve ordinal depth estimation and create a stronger impression of realistic depth. 

\begin{figure}[h]
	\centering
		\includegraphics[width=\textwidth]{disparity_distortion_supplement.pdf}
		\caption{Simulated conditions for estimating disparity distortions caused by conventional stereo rendering (right). The amount of expected disparity distortion is expected to be zero for foveal vision and increasing in the periphery of the visual field (left). When converted to perceived depth distortion (center), the expected amount of distortion, even in the periphery, is negligible and perhaps imperceivable.}
		\label{fig:supp:disparity}
\end{figure}


==> sections/supplement_stereopreference.tex <==
% !TeX root = ../supplement.tex

\begin{figure}[t]
	\centering
		\includegraphics[width=\columnwidth]{user_study/preference_study.pdf}
		\caption{Subjective depth perception. We asked users to rank conventional rendering, ocular parallax rendering, and reversed ocular parallax rendering by how effective these modes are in conveying the 3D structure of the scene. Neither the monocular nor the binocular conditions show a significant effect for any of the scenes (top row).}
		\label{fig:preference}
\end{figure}

In addition to measuring the effect of ocular parallax rendering on egocentric depth perception with the blind reaching task, we were also interested in evaluating depth perception in a more subjective way and studying if reversing the parallax direction would affect the experience. To this end, we designed a user experiment that allowed users to rank three different rendering modes in multiple conditions: conventional rendering, ocular parallax rendering, and reversed ocular parallax rendering. We studied the subjective user perception of these modes in monocular and stereoscopic viewing conditions with three scenes each. These scenes show a city scene from near, middle, and far viewpoints with the distance between background and closest foreground object being 3~D, 2~D, and 1~D, respectively. For this study, we tested 16 users (age range, 22\textendash29, 5 female), of which one was excluded for not passing a standard Randot stereo vision test, and two others were excluded due to the eye tracker failing to track their pupils. For each scene viewpoint (\autoref{fig:preference}, top), users were shown each rendering mode for 20 seconds, after which they could switch between and rank the modes at will. The presentation order of the viewpoints and modes was randomized. Seven subjects started in the monocular condition, while six started in the binocular condition. Participants were encouraged to gaze around the scene liberally, although this instruction was not strictly enforced. Head pose tracking was disabled. Participants were asked to rank the three rendering modes based on how effective they were in conveying the 3D structure of the scene.

Results of the rankings are shown in \autoref{fig:preference}. On average, participants did not seem to think any particular mode conveyed the 3D structure of the scene better than others. A Friedman test was used to test for statistical significance, and no effect was found. Interestingly, almost all participants reported to have seen the effect during a post-study debriefing stating that they could see a change in perspective or viewing angle in the two ocular parallax modes. Many commented on observing noticeable latency (i.e., ``snapping'') in both ocular parallax modes, resulting in a reduced sense of immersion. The display and the eye tracking were verified to update correctly at 90~Hz and 120~Hz, respectively, resulting in a theoretical latency of about 20~ms. Note that this latency represents the state of the art of eye tracking technology available for head-mounted displays today. Given that our sensitivity to differential velocities is smaller than our minimum angle of resolution across the visual field~\cite{Mckee:84}, it seems as though significantly lower latency is required to fully remove noticeable jitter and delay between eye rotation and ocular parallax rendering.
